AgentSense: Virtual Sensor Data Generation Using LLM Agents in Simulated Home Environments

A major challenge in developing robust and generalizable Human Activity Recognition (HAR) systems for smart homes is the lack of large and diverse labeled datasets. Variations in home layouts, sensor configurations, and individual behaviors further exacerbate this issue. To address this, we leverage the idea of embodied AI agents -- virtual agents that perceive and act within simulated environments guided by internal world models. We introduce AgentSense, a virtual data generation pipeline in which agents live out daily routines in simulated smart homes, with behavior guided by Large Language Models (LLMs). The LLM generates diverse synthetic personas and realistic routines grounded in the environment, which are then decomposed into fine-grained actions. These actions are executed in an extended version of the VirtualHome simulator, which we augment with virtual ambient sensors that record the agents' activities. Our approach produces rich, privacy-preserving sensor data that reflects real-world diversity. We evaluate AgentSense on five real HAR datasets. Models pretrained on the generated data consistently outperform baselines, especially in low-resource settings. Furthermore, combining the generated virtual sensor data with a small amount of real data achieves performance comparable to training on full real-world datasets. These results highlight the potential of using LLM-guided embodied agents for scalable and cost-effective sensor data generation in HAR. Our code is publicly available at https://github.com/ZikangLeng/AgentSense.

==> figure/basic_vary_virtual.tex <==

\begin{figure}[t]
    \centering
    \begin{adjustbox}{width=1\linewidth, vspace=-0.3in}
        \includegraphics[scale=0.5]{figure/basic_vary_virtual_fig.pdf}
    \end{adjustbox}
    \caption{TDOST Basic model performance when different amount of virtual data are used for training. The amount of amount of real data stays the same.  }
    
    \label{fig:basic_vary_virtual}
\end{figure}

% \end{document}

==> figure/motion_sensor.tex <==

\begin{figure}[t]
    \centering
    \begin{adjustbox}{width=1\linewidth}
        \includegraphics[scale=0.75]{figure/motion_sensor_fig.pdf}
    \end{adjustbox}
    \caption{Overview of virtual motion sensor data generation. 
    An LLM-generated sequence of actions is executed by the X-VirtualHome simulator with motion sensors synthetically placed in each room.
    Metadata corresponding to the sensor event triggers, such as location and time of occurrence, is used for the modeling pipeline. 
    }
    \label{fig:motion sensor}
\end{figure}

% \end{document}

==> figure/node_vis.tex <==

\begin{figure}[t]
    \centering
    \begin{adjustbox}{width=1.0\linewidth, vspace=-0.3in}
        \includegraphics[scale=0.75]{figure/node_vis.png}
    \end{adjustbox}
    \caption{Virtual object and appliance door sensor data are generated by executing an LLM-generated sequence of actions in the X-VirtualHome simulator—with virtual object sensors and door sensors placed on specific objects—where elliptical nodes (annotated with an ID, a name, and, if applicable, a state) denote rooms or objects, labeled arrows indicate relationships (e.g., Inside, On, Facing), and sensor event metadata (object name and timestamp) is recorded for the modeling pipeline. The red nodes on the thrid steps marks the state change of the fridge and toaster after executinng the action sequence.
    }
    \label{fig:env graph}
\end{figure}

% \end{document}

==> sections/discussion/main.tex <==
\section{Discussion}
\label{discussion}
A key challenge in developing robust smart home-based HAR models is the lack of large-scale labeled datasets, further complicated by variations in home layouts, sensor setups, and individual behaviors. 
To address this, we introduce \textit{AgentSense}, a virtual data generation pipeline that uses LLMs to create diverse personas and routines, which are then executed in a simulated home instrumented with virtual sensors. 
This enables the generation of rich, diverse datasets that improve HAR model performance, particularly in settings where data is scarce. 
Models trained with our virtual data and minimal real data achieve performance on par with those trained on full datasets, demonstrating the potential of simulation-driven approaches to overcome data scarcity.

In the following section, we outline how insights gained from this work can inform future directions and detail the next steps in advancing our research.


\input{figure/layouts}

\subsection{Bridging the Domain Gap Between Real and Virtual Homes}
\label{discussion-domainGap}
We generated virtual sensor datasets from 22 distinct environments within the VirtualHome simulator. While diverse, none of these virtual environments precisely replicate the home layouts found in the real-world HAR datasets used for evaluation. As illustrated in Figure \ref{fig:layout_comparison}, a comparison between a VirtualHome environment and the Milan dataset reveals noticeable differences—Milan, for instance, includes more rooms and unique spaces such as an aisle. These discrepancies in layout introduce a domain gap between the virtual and real data. Despite this, our results show that incorporating virtual data significantly improves HAR model performance, even in the presence of this domain mismatch.

One promising future direction is to leverage the control offered by simulation to replicate the specific layout of a target home when needed. This enables personalization of HAR models for specific homes at virtually no additional cost. By generating layout-matched virtual sensor data, the model can be better adapted to the unique movement patterns and spatial transitions of that home.

Consider, for example, a newly instrumented smart home with no prior sensor data. Traditionally, HAR model development in such settings requires a "cold phase" \cite{hiremath2022bootstrapping}—a period of passive observation during which user activities are manually annotated to create labeled training data. By extending \textit{AgentSense}, this phase could be bypassed entirely. A simple video walkthrough of the home can be used to reconstruct a 3D model of the environment using tools like Meshroom \cite{alicevision2021mesh}. This model can then be imported into the simulator to generate virtual sensor data that matches the actual home layout. 
With this virtual data, an initial HAR model can be trained and deployed from day one, enabling activity recognition without the need for manual labeling or real-world data collection -- thus supporting the transition to the maintenance procedure for HAR in homes \cite{hiremath2024maintenance}.

\subsection{Optimizing Sensor Placement Through Virtual Data Simulation for HAR}
\label{discussion-optimizeSensor}
We generated virtual sensor data using motion sensors placed according to predefined rules, as detailed in Section~\ref{sec: motion sensor}. However, the sensor placement can be fully customized within the virtual environment. This flexibility is particularly useful for identifying optimal sensor configurations when instrumenting a new home with ambient sensors.
Consider a scenario in which a new home is to be equipped with sensors to support recognition of a specific set of user-desired activities. Rather than deploying sensors directly and relying on trial-and-error in the real world, one can first simulate various sensor layouts in the virtual environment. By generating virtual sensor data under different configurations and evaluating the resulting HAR model performance, the optimal sensor layout can be identified—defined as the configuration that yields the highest activity recognition accuracy. This approach enables cost-effective, large-scale experimentation without the time and expense associated with real-world sensor deployment.

\subsection{Extending to Multi-modal Data Generation in Simulated Home Environments:}
As described in Section~\ref{sec: X-Virtualhome}, the VirtualHome simulator supports the generation of multiple camera-based modalities, including RGB images, depth maps, semantic segmentation, and pose data. Our extended version enhances this capability by adding support for multiple ambient sensor data streams that are time-synchronized with these visual modalities.

Among these, pose and video data are especially valuable for sensor-based HAR, as they allow the integration of existing Pose2IMU and Video2IMU methods~\cite{kwon2020imutube, xiao2021, Uhlenberg2022mesh, Xia2022, kwon2021complex, leng2023benefitgenerativefoundationmodels, Leng2024emotion, Hwang2024wheel} to generate synchronized virtual accelerometer and gyroscope signals. In future work, we plan to jointly simulate these sensor modalities, leveraging LLM-based activity generation to create richly annotated, multi-modal datasets. Such simulation of synchronized ambient and wearable sensor streams would enable more comprehensive activity analysis—combining the contextual awareness of ambient sensors with the fine-grained motion tracking offered by wearables, particularly for activities of daily living~\cite{arrotta2021marble}.


\subsection{Future Work}
\label{discussion-futureWork}
Several avenues for future work directly connect to the work we presented in this paper. 
In what follows, we outline some of these future avenues.

\subsubsection{Exploring Alternative Large Language Models for Virtual Data Generation:} 
In this work, we utilize GPT-4o-mini  or various language generation tasks, including persona creation, high-level routine synthesis, and decomposition into low-level action sequences. 
This model offers near-zero cost for generating the required sequences. 
It can be substituted with other open-source LLMs such as DeepSeek \cite{liu2024deepseek}, Claude \cite{anthropic2024claude35}, Gemini \cite{team2023gemini}, or Llama \cite{patil2024review, naveed2023comprehensive, touvron2023llama}.
In future iterations, we plan to investigate how different LLMs influence the generated action sequences and how these variations affect the resulting virtual data in simulation environments.

While our multi-stage prompting procedure and activity annotations rely on LLM-generated outputs, one could argue that these may not fully capture the nuances of real-world, situated home environments. 
In future work, we will include a formal evaluation of LLM outputs by comparing them against real resident inputs of annotation sourced via Amazon Mechanical Turk \cite{patel2022proactive}, as successfully demonstrated in prior studies.

\subsubsection{Exploring Additional Pretraining Methods with Virtual Data}
In this work, we utilized the state-of-the-art TDOST framework to assess the benefits of incorporating virtual data into the Human Activity Recognition (HAR) pipeline. 
Low-level action sequences generated by LLMs were fed into the VirtualHome simulator, and the resulting sensor event triggers were encoded using the TDOST representation. 
Evaluation was conducted by pre-training on virtual data, followed by fine-tuning with a combination of virtual and real data. 
This setup was benchmarked against the standard TDOST pipeline, which has demonstrated strong performance in generalizable, layout-agnostic HAR—where home layouts and activity patterns differ between source and target homes.
To examine whether virtual data enhances generalization, we directly compared TDOST alone with TDOST pre-trained on virtual data. 
The improved performance in the pre-trained variant highlights the utility of synthetic data for building robust HAR systems. 
In future work, we plan to expand this analysis by incorporating traditional baselines, for example, the use of CASAS features \cite{cook2012casas, alam2012review} and exploring other self-supervised pre-training strategies \cite{chen2024utilizing, chen2024enhancing, Haresamudram2022ssl, haresamudram2021contrastive, oord2018representation}.

\subsubsection{Enhancing Coverage and Diversity in HAR through LLM-Generated Activities:}
A notable advantage of incorporating LLMs in the simulation pipeline is their ability to generate broad spectrum of plausible human activities, many of which align with real-world behaviors yet remain underrepresented in existing HAR datasets. 
While such datasets are typically constrained by a fixed set of annotated labels, actual human routines are significantly more varied and context-dependent.
LLMs, trained on diverse and expansive textual corpora, can implicitly capture this behavioral richness and often produce activities that, though missing from benchmark datasets, mirror everyday human actions. 
In our generation process, we observed such instances, where the LLM surfaced realistic sequences absent from the labeled datasets -- highlighting limitations in traditional data collection pipelines, which are often bound by cost or activity taxonomies. 

Conversely, we also noted that certain activities commonly found in benchmark datasets, such as `Watch\_TV' or `Enter\_Home', were occasionally overlooked in the LLM-generated routines. 
This suggests areas where the open-ended simulation process could benefit from more targeted prompting 
In future work, we aim to explicitly include such activities to ensure alignment with established datasets and achieve fuller coverage of both common (occurring in benchmarked datasets) and underrepresented behaviors. 




